The Unreasonable Effectiveness of Random Target Embeddings for Continuous-Output Neural Machine Translation

Continuous-output neural machine translation (CoNMT) replaces the discrete next-word prediction problem with an embedding prediction. The semantic structure of the target embedding space (i.e., closeness of related words) is intuitively believed to be crucial. We challenge this assumption and show that completely random output embeddings can outperform laboriously pretrained ones, especially on larger datasets. Further investigation shows this surprising effect is strongest for rare words, due to the geometry of their embeddings. We shed further light on this finding by designing a mixed strategy that combines random and pre-trained embeddings for different tokens.

==> scratch.tex <==

%where other probabilistic constructions are considered, 
%with following work considering other loss functions \citet{kumar}
%and embedding choices \citet{tokarchuk-niculae-2022-target}.


%e.g., word2vec~\cite{NIPS2013_9aa42b31}, fastetext~\cite{bojanowski2016enriching} or embeddings transferred from discrete Transformer model~\cite{tokarchuk-niculae-2022-target}. Contextualized embeddings~\citep{ethayarajh-2019-contextual} are rarely used since it would require additional language model inference passes for each training step. The main downside of the initialization from a pre-trained model is that it requires an external model to get the embeddings from. This is computationally expensive, especially if training the model from scratch for the target language is needed. Another problem is that pre-trained models come with specific dimensions and vocabulary and must be adapted for the task at hand.



Maximum likelihood training requires 

%\vn{vlad will work on this section; we should start with the loss. The matrix P is not defined and not needed, let's just talk about E.}
To train a distance-based continuous-output model, we must obtain mapping for each discrete token $y_i \in V$ in a target sentence to the continuous vector $\mathbf{u}_i$ and from the continuous vector back to the discrete token $y_i$. Let's assume we have a projection matrix $\mathbf{P}$, with dimensionality $|V| \times\ d$ where $d$ is the dimensionality of the vector space and $|V|$ is the size of the target NMT vocabulary. We say that each row $i$ of the matrix $\mathbf{P}$ corresponds the token $y_i$, and \textit{embeddings} of the token $y_i$ is equal to:  
%$$
%    \mathbf{E}(y_i) = \mathbf{P}_{i,:}\ \ \forall i \in {1,2,...,V}.
%$$

We adopt the continuous-output Transformer architecture described in ~\cite{tokarchuk-niculae-2022-target}. The number of trained parameters is reduced compared to the discrete model since the projection layer is not trained in a continuous-output Transformer. See more details about model architecture in Appendix~\ref{app:model fig} Loss function is a distance function between vectors $\mathbf{E}(y_i)$ and $\mathbf{h}$. We use cosine distance similar to previous works. 
%
%$$\mathcal{L}(\mathbf{E}(y_i),\mathbf{h})=d_\text{cos}(\mathbf{E}(y_i),\mathbf{h}) = 1-\frac{\langle\mathbf{h},\mathbf{E}(y_i)\rangle}{\|\mathbf{E}(y_i)\|\|\mathbf{h}\|}$$

In our work, we focus on the initialization of matrix $P$. A common way to initialize matrix $P$ is to utilize pre-trained word or subword embeddings~\cite{kumar2018von,tokarchuk-niculae-2022-target}, e.g., word2vec~\cite{NIPS2013_9aa42b31}, fastetext~\cite{bojanowski2016enriching} or embeddings transferred from discrete Transformer model~\cite{tokarchuk-niculae-2022-target}. Contextualized embeddings~\citep{ethayarajh-2019-contextual} are rarely used since it would require additional language model inference passes for each training step. The main downside of the initialization from a pre-trained model is that it requires an external model to get the embeddings from. This is computationally expensive, especially if training the model from scratch for the target language is needed. Another problem is that pre-trained models come with specific dimensions and vocabulary and must be adapted for the task at hand.

Instead of obtaining embeddings from an external model, we propose synthetically generating $\mathbf{P}$ by initializing it with random embeddings. The random embeddings do not carry any linguistically meaningful information like the semantic similarity between tokens in the vocabulary. This is a main characteristic of pre-trained embeddings, which is assumed to be essential for training continuous-output models. The random embeddings can be further fine-tuned jointly with the model~\cite{Li-2022-DiffusionLM}, but this can lead to the collapse of representation because the perfect solution is embeddings that are all equal to each other. Instead, these embeddings can be kept untrained during training, which prevents collapse. 

%challenges the assumption that meaningful distances between tokens play a major role in the continuous-output model's performance.
% \vn{I would just emphasize more that ``output embeddings'' have different properties and problems; but we have to be careful since it's common to use tied embeddings too}

% To get discrete tokens back from the continuous representation, we rely on the nearest neighbors search, similar to previous works~\cite{tokarchuk-niculae-2022-target, Li-2022-DiffusionLM, kumar2018von}. We calculate the distance between the model output vector $\mathbf{h}$ and each vector in the matrix $P$.
% \begin{equation}
%     \Tilde{y} = \argmax_{i \in V}\ d(\mathbf{h}, \bm{P}_{i,:})
% \end{equation}
% Given the autoregressive nature of the transformer decoder, we do rounding at each token generation step, so each successive step is conditioned on the predicted token rather than continuous representation.

